Input from the SND@LHC collaboration to the 2026 Update to the European Strategy for Particle Physics

By observing collider neutrino interactions of different flavours, the SND@LHC and Faser experiments have shown that the LHC can make interesting contributions to neutrino physics. This document summarizes why the SND@LHC Collaboration intends to continue taking data at the High Luminosity LHC (HL-LHC). The upgraded detector will instrument the regions of both the neutrino vertex and the magnetized calorimeter with silicon microstrips. The use of this technology will allow us to continue the physics program of the current SND@LHC detector with higher statistics. It will also offer new possibilities. For instance, the magnetization of the hadron calorimeter will enable the separation between neutrinos and antineutrinos. This could lead to the first direct observation of tau antineutrinos. The use of ultrafast timing layers will enable triggers to be sent to ATLAS, potentially allowing the identification of the charm quark pair that produced the neutrino interacting in the detector. Such tagging of the neutrino source would fulfill Pontecorvo original proposal of a tagged neutrino beam. The experiment will perform unique measurements with high energy neutrinos and will also provide a means to measure gluon parton distribution functions in a previously unexplored domain (Bjorkenx <10^-5). Furthermore, the technological advancements of the upgrade and the experience that will be gained in the areas of operation and data analysis will play a crucial role in the design of the neutrino detector for the SHiP experiment.

==> chapters/detector.tex <==
\section{Detector}
\label{sec:detector}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



==> chapters/executive.tex <==
\section*{\Large Executive Summary }
\addcontentsline{toc}{section}{Executive Summary}
\label{sec:executive}

SND@LHC has been taking data since the beginning of the LHC RUN3, in 2022. The first publication, concerning the observation of muon neutrinos interactions was in 2023~\cite{SNDLHC:2023pun} followed by the publication of the measurement of the flux of muons~\cite{SNDLHC:2023mib} which constitute the most important background source. Progressing towards measuring electron Neutrino and neutral current interactions, the collaboration published the observation of neutrino interactions without a muon in the final state~\cite{SNDLHC:2024qqb}.
The measured muon flux highlights the limitations of the SND@LHC neutrino target setup: emulsions reconstruction capabilities reach a limit after about 20~fb$^{-1}$: this makes running at High LUMI LHC impractical as the target emulsions would need too frequent replacement.
The proposal for the upgraded SND@HL-LHC detector is to silicon strip to equip the target and act as  vertex detector. Modules  of the CMS Tracker outer barrel that will be decommissioned after Run~3 have been offered to us by the CMS Collaboration.  The modules available from the decommissioning of the CMS tracker are sufficient also to be used as well as the active element of the Hadron Calorimeter, providing a highly granular sampling of the hadronic showers associated to the neutrino interaction. The hadron calorimeter becomes as well a tracking device able to reconstruct the muon tracks produced either in the muon neutrino interactions or the decay of the tau   lepton produced in the tau neutrino interaction. 
We also propose to magnetize the iron absorber of the Hadron calorimeter ( 1.8 T field) which will allow determining the momentum of the muons and their charge. We expect to have momentum resolution of $\approx$ 20\% at 1 TeV and correspondingly better than 4$\sigma$ charge identification. This will allow us to separate neutrinos from antineutrinos.
The upgrade will be complemented by the addition of four fast timing detector layers in the target that will  be used  to trigger the silicon detector and to possibly send a trigger to ATLAS for the tagging of the neutrino parent. 
The neutrino physics program is unique: our pseudorapidity range and detector technology enable the observation of all three neutrino flavors, as the neutrino source is dominated by charmed mesons. Beyond measuring neutrino cross sections in an unexplored energy range, it will allow, for the first time, a comprehensive assessment of lepton flavor universality in the neutrino sector.

Since the charm quarks producing these neutrinos originate from gluon-gluon fusion, we will probe gluon PDFs at very low Bjorken$x$ (below $10^{-5}$) . This region is particularly significant as it may reach the expected saturation of gluon distributions, known as the QCD glass condensate. Improving gluon distribution measurements at low $x$
will also enhance our understanding of atmospheric neutrinos—crucial for experiments studying extragalactic neutrinos, such as KM3NeT and IceCube—and refine jet production models in the endcap region of a potential future FCC-hh collider.













==> chapters/outlook.tex <==
\section{Outlook}
\label{sec:outlook}


\newpage 

